PNI : Industrial Anomaly Detection using Position and Neighborhood Information

Because anomalous samples cannot be used for training, many anomaly detection and localization methods use pre-trained networks and non-parametric modeling to estimate encoded feature distribution. However, these methods neglect the impact of position and neighborhood information on the distribution of normal features. To overcome this, we propose a new algorithm, \textbf{PNI}, which estimates the normal distribution using conditional probability given neighborhood features, modeled with a multi-layer perceptron network. Moreover, position information is utilized by creating a histogram of representative features at each position. Instead of simply resizing the anomaly map, the proposed method employs an additional refine network trained on synthetic anomaly images to better interpolate and account for the shape and edge of the input image. We conducted experiments on the MVTec AD benchmark dataset and achieved state-of-the-art performance, with \textbf{99.56\%} and \textbf{98.98\%} AUROC scores in anomaly detection and localization, respectively.

==> 06_acknowledgements.tex <==
\paragraph{Acknowledgments} \cancel{This work was supported by Gauss Labs.}

==> tables/ablation_result_v0.tex <==
\begin{table}[t]
\centering
\footnotesize
\addtolength{\tabcolsep}{-0.7pt}
\renewcommand{\arraystretch}{1.05}
\caption{The Ablation Results on MVTec AD.}
\vspace{-0.40cm}
\label{ablation_result}
\begin{tabular}{c|cc|cc}
\noalign{\smallskip}\noalign{\smallskip}\hline\hline
& \small{Neighbor} & \small{Position} & \small{Detection} & \small{Localization} \\
\hline
\hline
PatchCore & - & - & 99.06 & 98.05 \\
\hline
\multirow{3}{*}{\begin{tabular}{@{}c@{}}Proposed \\ (w/o refine)\end{tabular}} & o & x & 99.44 & 98.62 \\
 & x & o & 99.25 & 98.72 \\
 & o & o & 99.46 & 98.80 \\
\hline
Proposed & o & o & \textbf{99.56} & \textbf{98.99} \\
\hline
\hline
\end{tabular}
\vspace{-0.30cm}
\end{table}


==> tables/anomaly_performance_mvtecad_v0.tex <==
\begin{table*}[t]
\centering
\footnotesize
\addtolength{\tabcolsep}{1.9pt}
\renewcommand{\arraystretch}{1.05}
\caption{Anomaly Detection and localization AUROC score on MVTec AD. The first and the second numbers are detection and localization scores, respectively. We provided sub-total averages for object and texture type classes.}
\vspace{-0.40cm}
\label{anomaly_performance_mvtec}
\begin{tabular}{cl|cccc|cc}
\noalign{\smallskip}\noalign{\smallskip}\hline\hline
 
& 
& \small{CFLOW-AD \cite{gudovskiy2022cflow}} 
& \small{PatchCore \cite{roth2022towards}} 
& \begin{tabular}{@{}c@{}}\small{FastFlow \cite{yu2021fastflow}} \\ 

(WRN50)\end{tabular} 
& \begin{tabular}{@{}c@{}}FastFlow \\
(CaiT)\end{tabular} & \begin{tabular}{@{}c@{}}Proposed \\ (w/o refine)\end{tabular} & Proposed \\
\hline
\hline
\multirow{10}{*}{Object} 
& Bottle & \hspace{0.22cm}(\textbf{100}, 98.76) & (\textbf{100}, 98.6) & - & (\textbf{100}, 97.7) & \hspace{0.22cm}(\textbf{100}, 98.79) & \hspace{0.22cm}(\textbf{100}, \textbf{98.82}) \\
& Cable & (97.59, 97.64) & (99.5, 98.4) & - & (\textbf{100}, 98.4) & (99.43, 99.07) & (99.78, \textbf{99.08}) \\
& Capsule & (97.68, 98.98) & (98.1, 98.8) & - & (\textbf{100}, 99.1) & (99.44, 99.32) & (99.76, \textbf{99.33}) \\
& Hazelnut & (99.98, 98.82) & (\textbf{100}, 98.7) & - & (\textbf{100}, 99.1) & (\textbf{100}, 99.10) & \hspace{0.22cm}(\textbf{100}, \textbf{99.44}) \\
& Metal nut & (99.26, 98.56) & (\textbf{100}, 98.4) & - & (\textbf{100}, 98.5) & \hspace{0.22cm}(\textbf{100}, 99.29) & \hspace{0.22cm}(\textbf{100}, \textbf{99.30}) \\
& Pill & (96.82, 98.95) & (96.6, 97.1) & - & (\textbf{99.4}, \textbf{99.2}) & (96.97, 99.02) & (97.05, 99.05) \\
& Screw & (91.89, 98.10) & (98.1, 99.4) & - & (97.8, 99.4) & (\textbf{99.57}, 99.59) & (99.55, \textbf{99.60}) \\
& Toothbrush & (99.65, 98.56) & (\textbf{100}, 98.7) & - & (94.4, 98.9) & \hspace{0.22cm}(99.44, 99.01) & (\textbf{100}, \textbf{99.11}) \\
& Transistor & (95.21, 93.28) & (\textbf{100}, 96.3) & - & (99.8, 97.3) & \hspace{0.22cm}(\textbf{100}, 97.88) & \hspace{0.22cm}(\textbf{100}, \textbf{97.90}) \\
\hline
&  & (97.56, 97.96) & (99.14, 98.27) & - & (99.04, 98.62) & (99.43, 99.01) & (\textbf{99.57}, \textbf{99.07}) \\
\hline
\hline
\multirow{7}{*}{Texture} 
& Carpet & (98.73, 99.23) & (98.7, 99.0) & - & (\textbf{100}, 99.4) & (99.80, 99.27) & \hspace{0.22cm}(\textbf{100}, \textbf{99.41}) \\
& Grid & (99.60, 96.89) & (98.2, 98.7) & - & (\textbf{99.7}, 98.3) & (98.41, 98.99) & (98.41, \textbf{99.18}) \\
& Leather & \hspace{0.22cm}(\textbf{100}, \textbf{99.61}) & (\textbf{100}, 99.3) & - & (\textbf{100}, 99.5) & \hspace{0.22cm}(99.83, 99.49) & \hspace{0.22cm}(\textbf{100}, 99.60) \\
& Tile & (99.88, 97.71) & (98.7, 95.6) & - & (\textbf{100}, 96.3) & \hspace{0.22cm}(99.96, 97.64) & (99.96, \textbf{98.51}) \\
& Wood & (99.12, 94.49) & (99.2, 95.0) & - & (\textbf{100}, 97.0) & (99.30, 96.26) & (99.21, \textbf{97.08}) \\
& Zipper & (98.48, 98.41) & (98.8, 98.8) & - & (99.5, 98.7) & (\textbf{99.76}, 99.33) & (99.68, \textbf{99.38}) \\
\hline
&  & (99.30, 97.72) & (98.93, 97.72) & - & (\textbf{99.87}, 98.2) & (99.51, 98.50) & (99.54, \textbf{98.86}) \\
\hline
\hline
&  Average & (98.26, 97.87) & (99.06, 98.05) & (99.3, 98.1) & (99.37, 98.45) & (99.46, 98.80) & (\textbf{99.56}, \textbf{98.99}) \\
\hline
\hline
\end{tabular}
\vspace{-0.30cm}
\end{table*}


==> tables/btad_result_v0.tex <==
\begin{table}[h]
\centering
\footnotesize
\addtolength{\tabcolsep}{1.7pt}
\renewcommand{\arraystretch}{1.05}
\caption{Anomaly localization results on BTAD.}
\vspace{-0.40cm}
\label{btad_result}
\begin{tabular}{c|cc|cc}
\noalign{\smallskip}\noalign{\smallskip}\hline\hline
& \begin{tabular}{@{}c@{}}VT-ADL \\ \cite{mishra2021vt}\end{tabular} & \begin{tabular}{@{}c@{}}FastFlow \\ \cite{yu2021fastflow}\end{tabular} & \begin{tabular}{@{}c@{}}Proposed \\ (w/o refine)\end{tabular} & Proposed\\
\hline
\hline
1 & \textbf{99} & 95 & 97.0 & 97.4\\
2 & 94 & 96 & 96.5 & \textbf{96.6}\\
3 & 77 & 99 & 98.9 & \textbf{99.1}\\
\hline
\hline
Average & 90.0 & 96.7 & 97.5 & \textbf{97.7}\\
\hline
\hline
\end{tabular}
\vspace{-0.30cm}
\end{table}


==> tables/ensemble_result.tex <==
\begin{table}[!t]
    \scriptsize
    \setlength{\tabcolsep}{20pt}
    % \renewcommand{\arraystretch}{1.05}
    \caption{The Ensemble Results on MVTec AD.}
    \vspace*{-0.2cm}
    \centering
    \begin{tabular}{c|cc}
    \toprule
                & I-AUROC & P-AUROC \\
    \midrule
    CFLOW-AD~\cite{gudovskiy2022cflow}  & 94.60 & 98.62 \\
    PatchCore~\cite{roth2022towards}    & 99.6 & 98.2 \\
    FastFlow~\cite{yu2021fastflow}      & 99.4 & 98.5 \\
    Proposed                            & \textbf{99.63} & \textbf{99.06} \\
    \bottomrule
    \end{tabular}   
    \label{tb:ensemble_result}
    \vspace*{-0.2cm}
\end{table}

==> tables/ensemble_result_v0.tex <==
\begin{table}[h]
\centering
\footnotesize
\addtolength{\tabcolsep}{12.0pt}
\renewcommand{\arraystretch}{1.05}
\vspace{-0.10cm}
\caption{The Ensemble Results on MVTec AD.}
\vspace{-0.40cm}
\label{ensemble_result}
\begin{tabular}{c|cc}
\noalign{\smallskip}\noalign{\smallskip}\hline\hline
& \small{Detection} & \small{Localization} \\
\hline
\hline
CFLOW-AD & 94.60 & 98.62 \\
PatchCore & 99.6 & 98.2 \\
FastFlow & 99.37 & 98.45 \\
\hline
Proposed & \textbf{99.62} & \textbf{99.06} \\
\hline
\hline
\end{tabular}
\vspace{-0.20cm}
\end{table}

==> tables/stc_result.tex <==
\begin{table}[]
\centering
\footnotesize
\addtolength{\tabcolsep}{2.4pt}
\renewcommand{\arraystretch}{1.05}
\caption{Anomaly localization performance on mSTC}
\vspace{-0.40cm}
\label{stc_result}
\begin{tabular}{cccc|c}
\noalign{\smallskip}\noalign{\smallskip}\hline\hline
CAVGA 
& SPADE 
& PaDiM 
& PatchCore 
& Proposed \\

\cite{attention_guided} 
& \cite{spade} 
& \cite{padim} 
& \cite{patchcore} 
& (w/o refine) \\

\hline
\hline
85 & 89.9 & 91.2 & 91.8 & \textbf{92.5} \\
\hline
\hline
\end{tabular}
\vspace{-0.30cm}
\end{table}
